Unlocking Scientific Concepts: How Effective Are LLM-Generated Analogies for Student Understanding and Classroom Practice?

Teaching scientific concepts is essential but challenging, and analogies help students connect new concepts to familiar ideas. Advancements in large language models (LLMs) enable generating analogies, yet their effectiveness in education remains underexplored. In this paper, we first conducted a two-stage study involving high school students and teachers to assess the effectiveness of LLM-generated analogies in biology and physics through a controlled in-class test and a classroom field study. Test results suggested that LLM-generated analogies could enhance student understanding particularly in biology, but require teachers' guidance to prevent over-reliance and overconfidence. Classroom experiments suggested that teachers could refine LLM-generated analogies to their satisfaction and inspire new analogies from generated ones, encouraged by positive classroom feedback and homework performance boosts. Based on findings, we developed and evaluated a practical system to help teachers generate and refine teaching analogies. We discussed future directions for developing and evaluating LLM-supported teaching and learning by analogy.

==> list/plain_generation.tex <==

%\captionsetup[lstlisting]{position=bottom}
\lstset{
    backgroundcolor=\color[RGB]{245,245,244},
    breaklines=true,
    breakindent=0pt,
    basicstyle=\ttfamily\small,
    %emph={Structure,Analogy,Free,Form,Word,Generation,Concept},
    emphstyle={\bfseries\color{NavyBlue}}
}\begin{lstlisting}[caption={Prompt templates for GPT-4 to generate analogies.},label=lst:analogy_generation_prompt]
Your task is to use an analogy to explain the scientific concept to students. 
Here are some principles for generating appropriate analogies:

1. The similarity between the objects in the analogy and those in the scientific concept should be minimal.
2. The relationships in the analogy and the scientific concept should be highly similar.
3. The analogy should use objects that students are very familiar with from everyday experiences.

To generate the appropriate analogy according to students' learning progress, we provide you with textbook content related to this scientific concept for your reference.
The textbook content: {input_text}
The scientific concept: {concept}
Analogy (Answer in Chinese):
\end{lstlisting}

==> list/revised_generation.tex <==

%\captionsetup[lstlisting]{position=bottom}
\lstset{
    backgroundcolor=\color[RGB]{245,245,244},
    breaklines=true,
    breakindent=0pt,
    basicstyle=\ttfamily\small,
    %emph={Structure,Analogy,Free,Form,Word,Generation,Concept},
    emphstyle={\bfseries\color{NavyBlue}}
}\begin{lstlisting}[caption={The revised prompt templates for GPT-4 to generate analogies.},label=lst:analogy_generation_prompt_revise]
Your task is to use an analogy to explain the scientific concept to students. 
Here are some principles for generating appropriate analogies:

1. The objects in the analogy and the scientific concept should align with scientific laws and commonsense knowledge.
2. The similarity between the objects in the analogy and those in the scientific concept should be minimal.
3. The relationships in the analogy and the scientific concept should be highly similar.
4. The analogy should accurately identify similar relationships with the scientific concept and avoid forcing non-existent similarities.
5. The analogy should use objects that students are very familiar with from everyday experiences.
6. An object in the analogy cannot have different roles or functions in different contexts.
7. The logic within a sentence or paragraph should not be self-contradictory.

To generate the appropriate analogy according to students' learning progress, we provide you with textbook content related to this scientific concept for your reference.
The textbook content: {input_text}
The scientific concept: {concept}
Analogy (Answer in Chinese):
\end{lstlisting}

==> table/findings_in_study2_pre_class_interview.tex <==
\begin{small}
\begin{longtable}[t]
{@{}p{0.2\linewidth}p{0.39\linewidth}p{0.39\linewidth}@{}}
\caption{A Summary of Interviewing Physics and Biology Teachers.} \label{tab:findings_in_study2_pre_class_interview}\\
\toprule
\textbf{Topic} & \textbf{Physics Teacher (T1)} & \textbf{Biology Teacher (T2)} \\ 
\midrule
\endfirsthead

\multicolumn{3}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\toprule
\textbf{Topic} & \textbf{Physics Teacher (T1)} & \textbf{Biology Teacher (T2)} \\
\midrule
\endhead

\bottomrule
\endfoot

\bottomrule
\endlastfoot

\rowcolor[gray]{0.95}\multicolumn{3}{c}{\textbf{Analogy Usage Exploration}} \\
Analogies Frequency & Sometimes. & Frequent. \\
\midrule
Analogies Feature & Mostly between learned concepts. & Mostly between biology and daily life. \\
\midrule
Source of Analogies & Mostly Prepared analogies between concepts. \newline A few improvised analogies with everyday lives. & Mostly prepared analogies. \newline Nearly no improvised analogies. \\
\midrule
Good Analogy Criterion & Easy to understand and free of scientific errors. & Easy to understand and related to everyday life. \\
\midrule
Agreement with Initial Principles in Study I & Partial agreement: Analogies between similar physical concepts. & Total Agreement. \\
\midrule
Analogy Explanation & Verbal explanation + imagery + teaching aids & Verbal explanation + imagery + teaching aids \\
\midrule
Analogies Usage Scenario & Often used to introduce concepts. \newline Sometimes throughout teaching to help students remember key points & Often used when detailing knowledge points. \\
\midrule
Agreement with the Six-step Model of Practice~\cite{richland_analogy_2015} & Acknowledges most, except for pointing out differences when introducing concepts. & Totally agreement. \\
\midrule
Student Participation in Constructing Analogies & Rare. Sometimes, students offer their ideas, which might be used in the next class. & Rare. Sometimes, students prepare analogies for student-led discussions. \\
\midrule
Students Understanding Examination & Question students with "Have you seen something similar before?", or observe students' expressions & Students complete a few exercises during class, or question students about concept differentiation. \\
\midrule
\rowcolor[gray]{0.95}\multicolumn{3}{c}{\textbf{AI Usage Exploration}} \\
Awareness and Experience with AI & Has used ChatGPT for writing papers, lesson plans, and creating images; knows about Sora. & Has used ChatGPT for tenders and personal use. \\
\midrule
Pros and Cons of AI & Pros: helps write unexpected things. \newline Cons: Needs specific questions; AI usually doesn't follow the instructions. & Pros: Provides broad ideas.  \newline No clear cons due to limited experience. \\
\midrule
Can AI Replace Teachers? & Teachers know students' learning situations, AI does not; AI-generated content needs adjustment. & AI cannot replace but complement teachers. \\
\midrule
\rowcolor[gray]{0.95}\multicolumn{3}{c}{\textbf{Expectations Sharing on LLM-generated Analogies}} \\
Positive Comments on Analogies in Study I & 1. The analogies are all vivid and some of them are interesting & 1. Some analogies are similar to those used in class \newline 2. Identify analogies to try in class for concepts not usually taught with analogies. \\
\midrule
Negative Comments on Analogies in Study I & 1. Analogies don't clarify abstract concepts. \newline 2. Analogies can complicate simple concepts. \newline 3. For concepts that are tested simply, memorization is enough. \newline 4. Pictures could make some concepts clear without analogies. & 1. Analogies shouldn't reflect all but the main concepts; the rest relies on memory. \newline 2. Pictures and animations can visualize familiar organisms without analogies. \newline 3. Although rare, related concepts sometimes are used as analogies. \\
\midrule
Overall Expectations & Vivid analogies between physical concepts. & Analogies from daily life for teaching focus; \newline Interesting analogies to stimulate learning interest.\\
\end{longtable}
\end{small}

==> table/latex_only_table_prompt.tex <==
\begin{table*}[t]
\footnotesize
  \centering
  \caption{\chifinal{Prompt template for GPT-4 to generate analogies (I) and select the analogy from three candidates for the given concept (II).
  {\color[rgb]{0,0.39,0}{\textit{Green texts}}} are new principle after revising.}
  }
    \begin{tabularx}{0.9\linewidth}{X}
    \toprule
    
    \rowcolor[gray]{0.95}\multicolumn{1}{c}{\textbf{I: Analogy Generation with Revised Prompt}} \\
    \midrule
    \makecell[l]{\color{gray}{/* \textit{Task Description} */}\\
    Your task is to use an analogy to explain the scientific concept to students. \\
    Here are some principles for generating appropriate analogies: \\
    \color{gray}{/* \textit{Principles} */}\\
    1. The similarity between the objects in the analogy and those in the scientific concept should be minimal.\\
    2. The relationships in the analogy and the scientific concept should be highly similar.\\
    3. The analogy should use objects that students are very familiar with from everyday experiences.\\
    \color[rgb]{0,0.39,0}{\textit{4. The analogy should accurately identify similar relationships with the scientific concept and avoid forcing non-existent similarities.}}\\
    \color[rgb]{0,0.39,0}{\textit{5. The objects in the analogy and the scientific concept should align with scientific laws and commonsense knowledge.}}\\
    \color[rgb]{0,0.39,0}{\textit{6. An object in the analogy cannot have different roles or functions in different contexts.}}\\
    \color[rgb]{0,0.39,0}{\textit{7. The logic within a sentence or paragraph should not be self-contradictory.}}\\
    \color{gray}{/* \textit{Input Resource} */}\\
    To generate the appropriate analogy according to students' learning progress, we provide you with textbook content related to this scientific concept\\ for your reference.\\
    The textbook content: \texttt{\{input\_text\}}\\
    The scientific concept: \texttt{\{concept\}}\\
    Analogy:
     }\\
     \midrule
     \rowcolor[gray]{0.95}\multicolumn{1}{c}{\textbf{II: Analogy Selection}} \\
    \midrule
    \makecell[l]{\color{gray}{/* \textit{Task Description} */}\\
    There are three candidate analogies which are used to explain the scientific concept based on textbook content. Your task is to select the best analogy\\ from these three candidates. \\
    Here are some principles for generating appropriate analogies: \\
    \color{gray}{/* \textit{Principles} */}\\
    \color{gray}{Same as principles in I (Omit)}\\
    \color{gray}{/* \textit{Input Resource} */}\\
    The textbook content: \texttt{\{input\_text\}}\\
    The scientific concept: \texttt{\{concept\}}\\
    The generated analogies: \\
    Candidate 1: \texttt{\{analogy\_1\}}\\
    Candidate 2: \texttt{\{analogy\_2\}}\\
    Candidate 3: \texttt{\{analogy\_3\}}\\
    You need to give reasons first and then give the answer with the format: \texttt{Final Answer: Candidate X} \\
    Answer:
     }\\
    \bottomrule
    \end{tabularx}
  \label{tab:instruction_prompt}
\end{table*}
